Women's Participation in Open Source Software: A Survey of the Literature

Participation of women in Open Source Software (OSS) is very unbalanced, despite various efforts to improve diversity. This is concerning not only because women do not get the chance of career and skill developments afforded by OSS, but also because OSS projects suffer from a lack of diversity of thoughts because of a lack of diversity in their projects. Studies that characterize women's participation and investigate how to attract and retain women are spread across multiple fields, including information systems, software engineering, and social science. This paper systematically maps, aggregates, and synthesizes the state-of-the-art on women's participation in Open Source Software. It focuses on women's representation and the demographics of women who contribute to OSS, how they contribute, the acceptance rates of their contributions, their motivations and challenges, and strategies employed by communities to attract and retain women. We identified 51 articles (published between 2005 and 2021) that investigate women's participation in OSS. According to the literature, women represent about 9.8\% of OSS contributors; most of them are recent contributors, 20-37 years old, devote less than 5h/week to OSS, and make both non-code and code contributions. Only 5\% of projects have women as core developers, and women author less than 5\% of pull-requests but have similar or even higher rates of merge acceptance than men. Besides learning new skills and altruism, reciprocity and kinship are motivations especially relevant for women but can leave if they are not compensated for their contributions. Women's challenges are mainly social, including lack of peer parity and non-inclusive communication from a toxic culture. The literature reports ten strategies, which were mapped to six of the seven challenges. Based on these results, we provide guidelines for future research and practice.

==> Tables/comparison_canedo.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\centering
%\scriptsize
\caption{Comparison between the Canedo et al. \cite{PS43}'s SLR and the present study}
\label{tab:comparison}

\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{{Canedo et al. \cite{PS43}'s study}}}                                                                                                                                                                                                                                                        & \multicolumn{2}{c|}{\textbf{Our study}}                                                                                                                                                                                                                    \\ \hline
\textsc{\begin{tabular}[c]{@{}l@{}}The possible problems causing women’s lack of interest\\ in the area of software development\end{tabular}}                                                                                                                                                                                             & \multicolumn{2}{l|}{\textsc{Challenges faced by women in OSS projects} \ref{sec:rq6}}                                                                                                                                                     \\ \hline
Prejudice and discrimination based on the gender                                                                                                                                                                                                                                                                                 & \multicolumn{2}{l|}{Toxic Culture}                                                                                                                                                                                                                \\ \hline
Women consider their performance unsatisfactory                                                                                                                                                                                                                                                                                  & \multicolumn{2}{l|}{Impostor Syndrome}                                                                                                                                                                                                            \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \multicolumn{2}{l|}{Lack of Peer Parity}                                                                                                                                                                                                          \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \multicolumn{2}{l|}{Non-Inclusive Communication}                                                                                                                                                                                                  \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \multicolumn{2}{l|}{Stereotyping}                                                                                                                                                                                                                 \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \multicolumn{2}{l|}{Community Reception Issues}                                                                                                                                                                                                   \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \multicolumn{2}{l|}{Work-Life Balance Issues}                                                                                                                                                                                                     \\ \hline
\textsc{\begin{tabular}[c]{@{}l@{}}The possible solutions to increase the engagement of \\ women in OSS projects\end{tabular}}                                                                                                                                                                                                           & 
\begin{tabular}[c]{@{}l@{}}Strategies to increase women's\\ participation in OSS (Section \ref{sec:rq7})\end{tabular} & \begin{tabular}[c]{@{}l@{}}Women's motivations to\\ participate in OSS \textbackslash{}ref\{sec:rq5\}\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Setting quotas for women {[}...{]} \\ \\ Stereotypes not created on the competence of this\\ group of professionals.\end{tabular}                                                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}Promote awareness of the presence\\ of peers\\ De-Stereotype the OSS\\ contributor\end{tabular}   & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Initiatives to assist in the development of leadership \\ skills and technical performance of women can be \\ adopted\end{tabular}                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}Promote women to leadership\\ roles (empowerment)\end{tabular}                                    & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Transparency regarding the organizational\\ culture {[}...{]}\end{tabular}                                                                                                                                                                                                                            &                                                                                                                              & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \cline{1-1} \cline{3-3} 
The adoption of a code of conduct {[}...{]}                                                                                                                                                                                                                                                                                      &                                                                                                                              & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \cline{1-1} \cline{3-3} 
Anti-harassment policies and  active moderators {[}...{]}                                                                                                                                                                                                                                                                        & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Create and enforce a Code of\\ Conduct\end{tabular}}                             & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
Women’s support groups {[}...{]}                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Promote women-specific groups\\ and events\end{tabular}                                           & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Projects that are inserted in the context of Humanitarian \\ Free Open-Source  Software (HFOSS) {[}...{]} philanthropic\\ objectives, due to their altruistic nature, have been seen \\ as a way, not yet proven, to engage women, developers, \\ in open  software development projects\end{tabular} & \cellcolor[HTML]{EFEFEF}                                                                                                     & Altruism                                                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}The need to learn new skills has been pointed out as a\\ motivator for women to enter, engage and persist in the\\ world of OSS\end{tabular}                                                                                                                                                          & \cellcolor[HTML]{EFEFEF}                                                                                                     & Learning                                                                                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Continuous monitoring of female participation can be\\ used to generate metrics {[}...{]}\end{tabular}                                                                                                                                                                                                & \begin{tabular}[c]{@{}l@{}}Promote awareness of the presence\\ of peers\end{tabular}                                         & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & Promote inclusive language                                                                                                   & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Encourage and be welcoming to\\ women\end{tabular}                                                & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & De-bias tools                                                                                                                & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}Recognize women's achievement\\ (visibility)\end{tabular}                                         & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & Prepare mentors to guide women                                                                                               & \cellcolor[HTML]{EFEFEF}                                                                                           \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \cellcolor[HTML]{EFEFEF}                                                                                                     & Enjoyment and Fun                                                                                                  \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \cellcolor[HTML]{EFEFEF}                                                                                                     & Kinship                                                                                                            \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \cellcolor[HTML]{EFEFEF}                                                                                                     & Ideology                                                                                                           \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \cellcolor[HTML]{EFEFEF}                                                                                                     & Career                                                                                                             \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \cellcolor[HTML]{EFEFEF}                                                                                                     & Pay                                                                                                                \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \cellcolor[HTML]{EFEFEF}                                                                                                     & Own-Use                                                                                                            \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \cellcolor[HTML]{EFEFEF}                                                                                                     & Reciprocity                                                                                                        \\ \hline
\cellcolor[HTML]{EFEFEF}                                                                                                                                                                                                                                                                                                         & \cellcolor[HTML]{EFEFEF}                                                                                                     & Reputation                                                                                                         \\ \hline
\end{tabular}
\end{table*}

==> Tables/list_of_primary_studies.tex <==
\begin{table*}[htb]
\centering
%\scriptsize
\caption{Research questions and the respective primary studies that provide data to answer them}
\label{tab:primary_studies}
\begin{tabular}{l|l}
\toprule

\textbf{ID} & \textbf{RQs} \\ \hline

\cite{PS1} & RQ1, RQ5

\\ \hline

\cite{PS2} & RQ1, RQ2, RQ4            

\\ \hline
\cite{PS3} & RQ1, RQ3, RQ6   

\\ \hline

\cite{PS4} & RQ1, RQ2

\\ \hline

\cite{PS5} & RQ1, RQ2, RQ4

\\ \hline

\cite{PS6} & RQ1, RQ2, RQ6

\\ \hline

\cite{PS7} & RQ1       

\\ \hline
\cite{PS8} & RQ1, RQ6 

\\ \hline

\cite{PS9} & RQ1, RQ2, RQ6

\\ \hline
\cite{PS10} & RQ2

\\ \hline

\cite{PS11} & RQ2

\\ \hline
\cite{PS12} & RQ1, RQ2, RQ6

\\ \hline

\cite{PS13} & RQ2, RQ5

\\ \hline

\cite{PS14} & RQ2 

\\ \hline

\cite{PS15} & RQ2

\\ \hline

\cite{PS16} & RQ1, RQ4, RQ6

\\ \hline

\cite{PS17} & RQ1 

\\ \hline

\cite{PS18} & RQ4, RQ5 

\\ \hline

\cite{PS19} & RQ4  

\\ \hline

\cite{PS20} & RQ5  

\\ \hline

\cite{PS21} & RQ1, RQ5, RQ6 

\\ \hline

\cite{PS22} & RQ5 

\\ \hline

\cite{PS23} & RQ5, RQ6 

\\ \hline

\cite{PS24} & RQ5, RQ6 

\\ \hline

\cite{PS25} & RQ5, RQ6 

\\ \hline

\cite{PS26} & RQ5, RQ6 

\\ \hline

\cite{PS27} & RQ5, RQ6            

\\ \hline

\cite{PS28} & RQ1, RQ5, RQ6

\\ \hline

\cite{PS29} & RQ6

\\ \hline

\cite{PS30} & RQ6

\\ \hline

\cite{PS31} & RQ6

\\ \hline

\cite{PS32} & RQ6

\\ \hline

\cite{PS33} & RQ6

\\ \hline

\cite{PS34} & RQ6           

\\ \hline

\cite{PS35} & RQ6   

\\ \hline

\cite{PS36} & RQ6

\\ \hline

\cite{PS37} & RQ6

\\ \hline

\cite{PS38} & RQ6

\\ \hline

\cite{PS39} & RQ6       

\\ \hline

\cite{PS40} & RQ6

\\ \hline

\cite{PS41} & RQ6

\\ \hline

\cite{PS42} & RQ6

\\ \hline

\cite{PS43} & RQ1

\\ \hline

\cite{PS44} & RQ1

\\ \hline

\cite{PS45} & RQ2

\\ \hline

\cite{PS46} & RQ2

\\ \hline

\cite{PS47} & RQ6

\\ \hline

\cite{PS48} & RQ6

\\ \bottomrule
\end{tabular}
\end{table*}

==> Tables/quality_criteria.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\caption{Quality Assessment Checklist}
\label{tab:quality_criteria}
\begin{tabular}{l|l}
\hline
Q1  & Does the paper state its aim (e.g., objectives, research goal, focus)? (1. No, 2. Yes)                                                                         \\ \hline
Q2  & Does the paper position itself within existing literature? (1. No, 2. Yes)                                                                                     \\ \hline
Q3  & What is the study design? (1. Empiric; 2. Experience report; 3. Theoretical)                                                                                   \\ \hline
Q4 &
  \begin{tabular}[c]{@{}l@{}}What were the scientific methods used to evaluate the proposed methods, techniques or tools? \\ (1. None; 2. Example; 3. Experience; 4. Evaluation with feasibility and pilot studies; 5. Analysis)\end{tabular} \\ \hline
Q5  & \begin{tabular}[c]{@{}l@{}}What research methods are used by the paper? (1. None; 2. Survey; 3. Action research; 4. Case study; 5. Experiment)\end{tabular} \\ \hline
Q6 &
  \begin{tabular}[c]{@{}l@{}}Which describes best the paper? (1. Reports an experience; 2. Reports an opinion without fundamental research; 3. Proposes a method, technique or tool; \\ 4. Proposes and uses a method, technique or tool in academia; 5. Proposes and uses a method, technique or tool in one OSS community/project;  \\ 6. Proposes and uses a method, technique or tool in more than one OSS community/project)\end{tabular} \\ \hline
Q7  & Were the findings or conclusion reported? (1. No, 2. Yes)                                                                                                      \\ \hline
Q8  & Was the data collection method(s) reported? (1. No, 2. Yes)                                                                                                    \\ \hline
Q9  & Was the data analysis method(s) reported? (1. No, 2. Yes)                                                                                                      \\ \hline
Q10 & Were limitations or threats to validity described? (1. No, 2. Yes)                                                                                             \\ \hline
\end{tabular}
\end{table*}

==> Tables/rq1_data.tex <==
\begin{table}[htb]
\centering
%\scriptsize
	\caption{Descriptive statistics of women's participation reported by primary studies}
	\label{tab:educ_level}
	{
		\begin{tabular}{l|r}
			\toprule
			 & \% Women  \\
			\cmidrule[0.4pt]{1-2}
			Mean & 9.114  \\ \hline
			Median & 9.750  \\ \hline
			Mode & 10.000  \\ \hline
			Std. Deviation & 2.654  \\ \hline
			Minimum & 4.300  \\ \hline
			Maximum & 14.200  \\ \hline
			25th percentile & 7.525  \\ \hline
			50th percentile & 9.750  \\ \hline
			75th percentile & 10.775  \\ 
			\bottomrule
		\end{tabular}
	}
\end{table}


==> Tables/rq1_education_level.tex <==
\begin{table}[htb]
	\centering
	%\scriptsize
	\caption{Education Level of Women who Contribute to OSS}
	\label{tab:educationlevel}
	{
		\begin{tabular}{l|r|r}
			\toprule
			 & Undergraduate or more & Ph.D  \\
			\cmidrule[0.4pt]{1-3}
			Mean & 80.440 & 12.300  \\ \hline
			Std. Deviation & 2.978 & 9.658  \\ \hline
			Minimum & 77.100 & 4.000  \\ \hline
			Maximum & 82.820 & 22.900  \\
			\bottomrule
		\end{tabular}
	}
\end{table}


==> Tables/rq1_frequency_of_women_old.tex <==
\begin{table}[htb]
\centering
%\scriptsize
\caption{Frequency of women's participation in OSS as reported by primary studies (ordered by year)}
\label{tab:frequency_old}
\begin{tabular}{l|r}
\toprule
Measure & Women \\ \hline
OSS contributors - survey (2013) \cite{PS2,PS5} & 10.4\%  \\ \hline
Participation in Wordpress mailing lists (2014) \cite{PS49} & 7.8\%  \\ \hline
Participation in Drupal mailing lists (2014) \cite{PS49} & 9.8\%  \\ \hline
Authors of Pull-Requests (2015) \cite{PS10} & 4.5\%   \\ \hline
GitHub users (2015) \cite{PS17} & 9.0\%   \\ \hline
GSoC mentors 2016 \cite{PS43} & 7.8\%  \\ \hline
GSoC students 2016 \cite{PS43} & 11.9\%  \\ \hline
GSoC mentors (2017) \cite{PS43}                                                  & 11.9\%  \\ \hline
GSoC students (2017) \cite{PS43}                                                  & 13.4\%  \\ \hline
GitHub committers (2018)  \cite{PS16} & 5.9\%   \\ \hline
GitHub account owners (2018)  \cite{PS16} & 10.0\%  \\ \hline
OpenStack contributors (2018) \cite{PS12} & 10.0\%  \\ \hline
GSoC mentors (2018) \cite{PS43} & 10.9\%  \\ \hline
GSoC students (2018) \cite{PS43} & 14.2\%  \\ \hline
Core Developers (2019) \cite{PS9} & 4.3\%   \\ \hline
Authors of Pull-Requests (2019) \cite{PS3} & 6.3\%   \\ \hline
Non-Casual Coders (2019) \cite{PS9} & 6.7\%   \\ \hline
GitHub users (2019) \cite{PS46} & 9.7\%   \\ \hline
Authors of contributions to public code (2019) \cite{PS44} & 10.0\%  \\\hline
OSS contributors - survey (2019)  \cite{PS21} & 10.9\%  \\ \hline
OSS contributors - survey (2021)  \cite{PS51} & 7.6\%  \\

\bottomrule
\end{tabular}
\end{table}


\begin{table*}[htb]
\centering
%\scriptsize
\caption{Frequency of women's participation in OSS as reported by primary studies}
\label{tab:frequency}
\begin{tabular}{l|c}
\toprule

%\rowcolor[HTML]{EFEFEF} 
\textbf{Data Source and Collection}                                          & \textbf{\% Women} \\ \hline
\multicolumn{2}{c}{\textbf{Mining}}                                                            \\ \hline
\multicolumn{2}{l}{{\textbf{GitHub}}}                                                      \\ \hline
\multicolumn{2}{l}{\textbf{* Users}}                                                           \\ \hline
GitHub users (2015) \cite{PS17}                             & 9                 \\ \hline
GitHub users (2019) \cite{PS46}                             & 9,7               \\ \hline
GitHub account owners (2018) \cite{PS16}                    & 10                \\ \hline
\multicolumn{2}{l}{\textbf{* Pull-Requests authors}}                                           \\ \hline
Authors of Pull-Requests (2015) \cite{PS10}                 & 4,5               \\ \hline
Authors of Pull-Requests (2019) \cite{PS4}                  & 5,2               \\ \hline
Authors of Pull-Requests (2019) \cite{PS3}                  & 6,3               \\ \hline
Authors of contributions to public code (2019) \cite{PS44}  & 10                \\ \hline
\multicolumn{2}{l}{\textbf{* Commit authors}}                                                  \\ \hline
GitHub committers (2018) \cite{PS16}                        & 5.9\%             \\ \hline
Core Developers (2019) \cite{PS9}                           & 4.3\%             \\ \hline
Non-Casual Coders (2019) \cite{PS9}                         & 6.7\%             \\ \hline
OpenStack committers (2017) \cite{PS12}                     & 7.5\%             \\ \hline
\multicolumn{2}{l}{\textbf{* Code Review Submitters}}                                          \\ \hline
OpenStack code reviewers (2017) \cite{PS12}                 & 7.9\%             \\ \hline
\multicolumn{2}{l}{{\textbf{Mailing Lists}}}                                               \\ \hline
Participation in Wordpress mailing lists (2014) \cite{PS49} & 10.2\%            \\ \hline
Participation in Drupal mailing lists (2014) \cite{PS49}    & 8.5\%             \\ \hline
\multicolumn{2}{l}{{\textbf{Google Summer of Code}}}                                       \\ \hline
\multicolumn{2}{l}{\textbf{* Mentors}}                                                         \\ \hline
GSoC mentors (2016) \cite{PS43}                             & 7.8\%             \\ \hline
GSoC mentors (2017) \cite{PS43}                             & 11.9\%            \\ \hline
GSoC mentors (2018) \cite{PS43}                             & 10.9\%            \\ \hline
\multicolumn{2}{l}{\textbf{* Students}}                                                        \\ \hline
GSoC students (2016) \cite{PS43}                            & 11.9\%            \\ \hline
GSoC students (2017) \cite{PS43}                            & 13.4\%            \\ \hline
GSoC students (2018) \cite{PS43}                            & 14.2\%            \\ \hline
\multicolumn{2}{c}{\textbf{Survey}}                                                            \\ \hline
OSS contributors (2013)\cite{PS2,PS5}                       & 10.4\%            \\ \hline
OSS contributors (2019)\cite{PS21}                          & 10.9\%            \\ \hline
OSS contributors (2020)\cite{PS51}                          & 7.6\%             \\


\bottomrule
\end{tabular}
\end{table*}

==> Tables/rq2_data.tex <==
%----- Requires booktabs package -----%
\usepackage{booktabs}

\begin{table}[h]
	\centering
	\caption{Descriptive statistics of women's education level}
	\label{tab:educ_level}
	{
		\begin{tabular}{lrr}
			\toprule
			 & Undergraduate or more & Ph.D  \\
			\cmidrule[0.4pt]{1-3}
			Valid & 3 & 3  \\
			Missing & 0 & 0  \\
			Mean & 80.440 & 12.300  \\
			Std. Deviation & 2.978 & 9.658  \\
			Minimum & 77.100 & 4.000  \\
			Maximum & 82.820 & 22.900  \\
			25th percentile & 79.250 & 7.000  \\
			50th percentile & 81.400 & 10.000  \\
			75th percentile & 82.110 & 16.450  \\
			\bottomrule
		\end{tabular}
	}
\end{table}


==> not_used_text.tex <==
%This paper is organized as follows. The next section provides a brief primer on gender diversity in OSS projects. Section 3 describes this study’s research questions and method; that is, systematic mapping. We then present the findings in Section 4. Section 5 discusses the implications and limitations of our findings and offers avenues for future research. Section 6 concludes the paper with a summary of its contributions.

%The women's equality in all areas is positioned as one of the main goals  of organizations and governments. Global organizations such as the United Nations (UN) or UNESCO (United Nations Educational, Scientific and Cultural Organization) employ initiatives focused on promoting both gender equality and the empowerment of women. The new campaign of UN is called ``Generation Equality: Realizing women's rights for an equal future”, and concentrates on fundamental rights such as participation in decision-making, equal distribution of tasks and access to health services \cite{women2019generation}. Moreover, UNESCO has a project called SAGA (STEM - Science, Technology, Engineering, and Mathematics - And Gender Advancement) since 2015 to offer governments and policymakers a variety of tools to help reduce the current global gender gap in science, technology and engineering fields existing at all levels of education and research \cite{fernandez2016drives}. However, despite significant progress has been made in recent years, the rate of women in the STEM professions remains low. 

%We based our search string definition on the PICOC (Population-Intervention-Comparison-Outcome-Context) methodology \cite{petticrew2008systematic}. Our \textbf{population} is Women. Our \textbf{intervention} is their Participation. Since these might be of several types, such as available frequency of participation, the activities they perform, roles they play, challenges and barriers they face, the motivations they have to join, stay or leave, and the strategies that communities reported to attract, retain and increase their participation, we decided not to include their types in the search string, simply mapping all types found. Comparison is not usually performed in SMS, since the purpose of SMS is to map the available evidence when no conclusions can be reached. Our outcome is the results obtained by the intervention. Since our goal is to identify interventions and their results, we decided not to restrict the search to a specific type of outcome, simply mapping them as well. Our context is Open Source Software projects. Therefore, we defined our search string strongly based on the population and the context.

%\subsubsection{Unfiltered Search}

%\subsection{Quality Assessment}

%To evaluate the selected papers, we defined quality criteria by adapting and synthesizing multiple recommendations \cite{ivarsson2011method,kuhrmann2015software,dyba2007applying,shaw2003writing,kitchenham2004procedures} into a questionnaire of quality assessment criteria (Table \ref{tab:quality_criteria}). We adapted the criteria found in those studies to classify the identified papers.

%\input{Tables/quality_criteria}

%\section{Gender Diversity in Open Source Software - A Brief Primer}

%Diversity can arise from any attribute that differentiates people \cite{williams1998reilly}. Software development teams can be diverse in different ways, e.g., w.r.t. gender, experience levels, culture, role,  cognitive styles, personality, nationality, and coding language preference. A team can be more diverse in one attribute and less diverse in others. The diversity attributes may also be combined (e.g., in some cultures, women may face more barriers), which turns the analysis and the studies even more complex~\cite{vasilescu2015gender}.

%The relationship between team diversity and team outcomes has been previously investigated  \cite{horwitz2007effects,stahl2010unraveling}. A gender diverse software team brings different perspectives together, thus improving outcomes and being more productive \cite{vasilescu2015gender}.

%In OSS communities, which are comprised by collaborative and task-oriented groups, being geographic (and cultural) disperse is the standard, as contributors rarely meet in person. Instead, they  mobilize into online communities, and coordinate their activities through distributed communication channels (e.g., email lists, slack channels). Besides, OSS teams are dynamic, forming and dissolving organically according to the current task being worked in. Since OSS contributors are often volunteers, teams face high turnover \cite{robles2006contributor}. OSS communities usually have a core-periphery structure \cite{ducheneaut2005socialization}, in which a few developers comprise the core and drive the work, while a larger and less connected group of contributors comprise the periphery and supports the core by reporting issues, submitting patches or bringing documentation. Due to those characteristics, OSS teams have the interactions between members are typically limited to online channels, and it can be hard to precisely say who is part of a team and who is not. Diversity attributes may, therefore, perform differently in OSS than in offline groups \cite{martins2004virtual}.

%Demographic characteristics, such as gender, should be less salient in OSS \cite{riordan1997demographic}. This would also be supported by the fact that OSS communities typically function as meritocracies \cite{feller2000framework}, where sustained, high-quality contributions comprise the main drivers behind impression formation, reputation building, and trust \cite{bird2007open,dabbish2012social,marlow2013impression}.

%While Section \ref{sec} provides a more comprehensive understanding, women represent less than than 10\% of the OSS contributors \cite{david2008community,robles2014floss} because they face a lot of discrimination, and despite being knowledgeable, they often feel not being good enough (``impostor syndrome”). Some examples of social challenges that women's participation (and consequently the gender diversity) in OSS includes that communities are usually toxic and sexist \cite{nafus2012patches}, male-dominated and unfriendly for women \cite{vasilescu2014gender}.

%\textsc{Pull Request submitters:} Women represent only 4.54\% \cite{PS4} - 5\% \cite{PS10} of pull-requests' authors. However, when submitting pull-requests, women have at least 64\% of merge success rate \cite{PS4,PS10}, which is near to men's (63.87\%) \cite{PS4}. %Kofink \cite{PS10} analyzed 1.811.631 pull requests with determined gender information from 1.049.345 different users and found that female pull request contributions account for only 4.54\% of the total pull requests submitted in this data set. Terrell et al. \cite{PS4} presented a similar rate when found that women submitted 5\% of the pull-requests from the total 158.464 of pull-requests that gender could be identified. Additionally, according to authors, women are slightly less likely to submit a pull request that mentions an issue. Even not implying that women’s pull requests are less valuable, women's pull requests are less likely to fulfill an documented need. Based on the number of lines of code, modified files, and number of commits of the pull requests to evaluate the change's size, women make larger changes than men, in the sense that women's pull requests add and remove more lines of code, and contain more commits \cite{PS4}. 
%%%%

%\textbf{Meritocracy needs transparency, not unspoken rules.} 
%The basis concept of a governing structure built on meritocracy is to reward those who deliver, instead of voting or appointing the  leaders. While the meritocracy is seen to be a common form in OSS communities, it may also encourage negative aspects of competition within the community \cite{germonprez2014collectivism}.
%Hann et al. (2004) explore meritocracies in open source software communities of Apache developers and empirically demonstrate that “employers pay significantly higher wages to participants who attain a higher rank in the OSS community.” While this is an important finding for those individuals in the community, we need to understand more about the meaning of merit itself.
% Therefore, we fully recognise how broadly construed a meritocracy can be. It needs to include not just intellect and effort, but also values and sustainability. O’Mahony and Ferraro (2007) note: Contradicting a simplistic meritocratic explanation, developers who engaged in organization-building behaviors were more likely to become members of the leadership team. Thus, Debian may be a meritocracy, but merit is not measured solely by technical contribution. A prevalent assumption in research on open source software communities is that the contributions community members value the most are purely technical. Our study shows otherwise. In this community, the informal work of coordinating individual efforts and linking them to community goals became vital to leadership, particularly as the project matured. (p. 22)

%The FLOSS 2013 survey, in contrast to the original FLOSS survey from 2002, was open not only for OSS developers, but also to any other person who played any type of contributions to OSS projects. Therefore a question was included, where respondents could specify if they were mainly coders, performed other activities (such as documentation, translations, tests, artwork...) or both \cite{PS5}.

%Additionally, according to authors, women are slightly less likely to submit a pull request that mentions an issue. Even not implying that women’s pull requests are less valuable, women's pull requests are less likely to fulfill an documented need. Based on the number of lines of code, modified files, and number of commits in the pull requests, they found that women make larger changes than men \cite{PS4}. 

%\textbf{Strategies to increase women} Many companies, especially large ones, are actively trying to reduce the gender gap by holding events and sponsoring campaigns to encourage women to work in the software industry and to create a better workplace that is free from prejudice and discrimination. Examples of such initiatives include Microsoft’s Global Diversity and Inclusion program, Google’s Diversity campaign, and Mozilla’s Diversity and Inclusion Strategy. Bottom-up initiatives mostly started by women who already work in the software industry. Their main goal is to bring together women who are interested in information technology so that they can support each other. One example is a Facebook group called “Women in Tech,” which is followed by more than 1 million people. Numerous events are organized at universities to encourage women to choose a technical career path. The main goal of these gatherings is to show that the IT sector can be a friendly working environment \cite{blincoe2019perceptions}.

%Strategies are not fully implemented yet.
%The strategies mentioned by interviewees in \citet{P24}'s study to achieve a broader diversity were not completely implemented, only partial solutions, the creation of codes of conduct, events and communities exclusively for women to provide visibility of their  contributions. The participants from both Canedo et al. \cite{PS6} and \cite\PS8}'s studies made several suggestions how to make OSS more inclusive but authors did not mention if the actions were implemented in practice.

%% Altruism grows - While 37.17\% of the 226 surveyed women from FLOSS 2013 study joined to share knowledge and skills, almost the double rate (62.26\%) continued because of that altruistic motivation \cite{PS5}.

%%% Muitos challenges e poucas estratégias

%%% Sense of beloging in other domains
%\citet{pan2014heterogeneous} The sense of belonging was a predictor of engagement intention by women newcomers in open collaboration projects by a social identification.

%% MOTIVATIONS

%\textsc{Enjoyment and Fun.} Based on a set of interviews, Balali et al.~\cite{PS18} found that women contribute because they ``find it exciting.'' No women from Gerosa et al.'s~\cite{PS51} study reported that they joined OSS by fun and one continued for that.

%\textsc{Kinship.} While 38.85\% of the 226 women who answered the FLOSS survey joined to participate in new forms of cooperation, 31.45\% continued because of that~\cite{PS5}. Most (64\%) of the 23 women who answered a survey~\cite{PS16} select a project that has friends and colleagues. As part of kinship, peer parity also plays a role in women's motivation~\cite{PS50}. The authors found that social connections with other developers influence women's choices. No women from Gerosa et al.'s~\cite{PS51} study joined OSS by kinship and two continued for that.
 
%\textsc{Altruism.} While 37.17\% of the 226 women who took part in the FLOSS 2013 survey joined to share knowledge and skills, almost two times that amount (62.26\%) continued to contribute because of that altruistic motivation~\cite{PS5}. Still, from the same sample~\cite{PS5}, 21.24\% of women started to improve the OSS products of other developers. When analyzing 76 humanitarian OSS projects, Parra et al.~\cite{PS19} found that women are motivated to join this kind of OSS project to help people and having philanthropic objectives. No women from Gerosa et al.'s~\cite{PS51} study joined OSS by altruistic reasons, while 22\% (4 out of 18) continued for that.

%\textsc{Pay.} A survey conducted by Prana et al.~\cite{PS16} indicated that 64\% of the 23 women who answered the questionnaire are currently contributing because they are paid. Besides a motivation to stay, not being paid was mentioned by women interviewees from Balali et al.'s~\cite{PS18} study as a reason to leave when OSS ``is not their job''. Two women from Gerosa et al.'s~\cite{PS51} study joined OSS by pay-related reasons, and two (out of 18) continued for that.

%\textsc{Learning.} Most (67.70\%) of the 226 women who took part in the FLOSS 2013 survey joined to learn and develop new skills, 64.78\% continue because of that (S5)~\cite{PS5}. Two women from Gerosa et al.'s~\cite{PS51} study joined OSS to learn new skills, while three (out of 18) continued for that.

%\textsc{Own-Use.} David and Shapiro~\cite{PS50} found that women are motivated by employment-related needs to use. One third (6 out of 18) of the women who answered the Gerosa et al.'s~\cite{PS51} questionnaire joined OSS because of \emph{Own-Use}, which is in line with previous research that shows that women are more motivated to use technology for what it enables them to accomplish a given goal~\cite{burnett2010gender}.

%Previous studies have reviewed and investigated different aspects of the literature on Open Source Software (OSS): structure, adoption, technical, educational and social.

%% OSS Ecossystem %%%
%When analyzing the \textsc{structure} of OSS communities, Franco-Bedoya et al.~\cite{franco2017open} investigated the OSS as an ecossystem paradigm to understand dynamics and heterogeneity in collaborative software development. Authors consolidated the most relevant definitions, the types and how the knowledge is represented in OSS ecossystems.

%% OSS Adoption %%%
%On the \textsc{adoption} side, Lenarduzzi et al.~\cite{lenarduzzi2020open} investigated the factors considered by evaluation models when selecting OSS projects, which included functionality, economic, license, community and adoption, support and service, operational software characteristics, development process and quality. The adoption was also the goal of Hauge et al.'s~\cite{hauge2010adoption} study, that provided a classification framework of six distinctly different ways in which organizations adopt OSS: deploying OSS products, using OSS tools, integrating OSS components, participating in OSS communities, providing OSS products, and using OSS practices. One more categorization of the adoption of OSS components and development methodologies by the industry was provided by Host and Orucevic-Alagic~\cite{host2011systematic}: OSS as part of component based software engineering, business models with OSS in commercial organization, company participation in OSS development communities, and usage of OSS processes within a company.

%% OSS Software Development Models and Activities %%%
%Software quality is part of the \textsc{technical} factors that can influence OSS adoption, and was the main goal of Adewumi et al.'s~\cite{adewumi2016systematic} study, that classified the literature findings about quality assessment models into five categories based on the quality characteristics they possess namely: non-quality, single-attribute, rounded category, community-only attribute, and non-community attribute. According to the study, software selection based on hierarchical structures is the most popular selection method in the existing OSS quality assessment models, and the majority (47\%) of the existing models do not specify any domain of application. Acuna et al.~\cite{acuna2012systematic} investigated not only the quality but all the OSS development process to understand the groups of activities included in the OSS software development models. Authors classified the findings in Concept Exploration, Software Requirements, Design, Maintenance and Evaluation, and found that testing and conducting reviews were the more prominent activities in the OSS development processes, which along with quality, belong to the Evaluation activities group. Another stage of development process was focused by Wu et al.'s~\cite{wu2016maintenance} study, that presented the existing approaches to estimate maintenance effort for OSS, by actual effort and by maintenance activity time prediction. The metrics are mainly related to source code and people, and the main activity about predicting time is bug fixing.

%%% Use of OSS for education
%Nascimento et al.~\cite{nascimento2015open} studied the use of OSS in \textsc{education} and how OSS projects have been used to facilitate students’ learning of software engineering, and found that most studies focused on comprehensive software engineering courses, and found that in general, students participate producing software in predefined OSS projects. 

%%% Barriers to join and challenges to use OSS
%On the \textsc{social} side, Steinmacher et al.~\cite{steinmacher2015systematic} presented 15 different barriers that new contributors face to join OSS, grouped into five categories: social interaction, newcomers’ previous knowledge, finding a way to start, documentation, and technical hurdles. Documentation was also one of the six categories of the 21 challenges that Stol and Ali Babar~\cite{stol2010challenges} presented about integrating an OSS in product development. The other five categories were product selection, community support and maintenance, integration and architecture, migration and usage, legal and Business.

% As we presented in Section 4.1, women author less than 5\% of pull-requests. 
% The reduction from the participation in initial stages (e.g., as students of Google Summer of Code) to their representation as authors of pull requests can be a consequence of the several socio-cultural challenges faced by women during the process.
% As we presented in Section~\ref{sec:rq6}, even having similar or even higher rates of merge acceptance than men when they do not disclose their gender, women frequently report biases or lower acceptance rates when they explicitly identify themselves as women.
% According to the Onion Model, people start outside the project as readers and passive users; then move to the project periphery as bug fixers, bug reporters, peripheral developers, and active developers (developers without commit rights); and finally, enter the project as core members or project leaders \cite{nakakoji2002evolution}. 
% Although mentorship events enhance the participants' sense of competence and increase the chances of future contributions values~\cite{silva2020theory}, women are still not staying in F/OSS projects until they become code committers. 
%We consolidated the challenges and reasons to leave reported by the primary studies in Section \ref{sec:rq6}, and we could observe that most of them are socio-cultural nature, not related to technical skills. Indeed, as we presented in Section \ref{sec:rq6}, women have similar or even higher rates of merge acceptance than men. Besides the appropriate technical skills, Bosu and Sultana's study~\cite{PS9} suggested that women are as productive as their colleagues who are men in an inclusive F/OSS project, with some women developers showing more productivity than the average men developers.
%Even not supporting any inferences about whether men or women are more accurate at code review, results from Huang et al.~\cite{PS14}'s study indicates women present more reliable activity patterns.

%Enforcing the code of conduct among the project members can be one action to help mitigating the toxic culture~\cite{PS34}. The enforcement should include both reactive and proactive mechanisms. The  reactive mechanism can provide a process for contributors to denounce improper behavior and have rules to take actions against those who infringe the code. This can ultimately giving people the sense that the community does not tolerate toxic behavior. The proactive mechanism can monitor messages exchange, being supported by tools like bots~\cite{PS8, wessel2018power}, and educating contributors to avoid toxic and non-inclusive vocabulary.

%Situations that activate gender-STEM stereotypes hamper women’s interest and motivation in STEM and increase anxiety about their performance~\cite{beilock2007stereotype,cheryan2009ambient dasgupta2015female}. 
%Women tend to hide their identities and gender to avoid bias and protect themselves~\cite{PS1}, but not in women-specific spaces, demonstrating they felt safe and comfortable in these spaces~\cite{PS48}.

%Contributors often omit their gender to avoid being stereotyped, as mentioned by other participants of Ford et al.'s study~\cite{ford2019beyond}: ``I look for what I'm publishing, for if it tends to attract people into stereotyping me, then I omit to post my name/image, else I go for it.'' 

%Authors calculated and compared the marginal effects of behavioral gender for users with unknown gender and users who identify as women and found no advantage for hiding the gender. 

%The mind is so exquisitely attuned and nimble in selectively attending to stereotypical cues in one moment and then turning attention away quickly when the cue no longer exists. The allocation of attention occurs swiftly and automatically when individuals who are deeply invested in a performance domain encounter minimalistic cues signaling the gaze of a high-status member in a stereotyped domain~\cite{wu2020influence}.

%Women are disadvantaged (compared to men) in success (number of times other users have starred---bookmarked as applicable ---their repositories) due to their pattern of behavior, which means that women's disadvantage can happen more due to gendered behavior than to categorical discrimination~\cite{PS26}.


%In that sense, the strategies of \textsc{Promoting awareness about having other women} and \textsc{Recognizing women's achievement (visibility)} that we presented in Section~\ref{sec:rq7} can help to reduce the impostor syndrome that women reported to feel. The benefits of combining these two strategies are two-fold. While recognition support the retention of existent women, it also attracts new women who can see they can have similar success achieved by their peers. Those strategies have been applied in STEM and other domains. Publicizing success stories of women in STEM was a strategy used to attract more women in Latin America in STEM higher education programs~\cite{garcia2019engaging}. Establishing prizes and awards is a strategy that approximately 82\% of U.K. research institutions have applied to stimulate and attract more women in STEM~\cite{fatourou2019women}. In automotive industries, specific groups publish articles about women and recognize leading women personalities through e-news ~\cite{sultana2013women}. As in other domains, F/OSS projects should implement different mechanisms to reward and promote awareness of women, motivating them to stick around.

% Women join GSoC but are low represented as authors of code commits. Challenges and acceptance rates show they face socio-cultural challenges, instead of lacking in technical skills.

%\textbf{Women are as efficient as men... maybe even more.} Based on the two code contribution metrics (i.e., code churn per month and code changes per month), Bosu and Sultana's~\cite{PS9} evidenced the absence of significant differences when comparing men and women developers in terms of productivity. Moreover, the authors suggest that women are as productive as their male colleagues in an inclusive F/OSS project, with some women developers demonstrating more productivity than the average men developers. Even not supporting any inferences about whether men or women are more accurate at code review, results from Huang et al.~\cite{PS14}'s study indicates women present more reliable activity patterns. 

%\textbf{Women-specific spaces.} When offering women-only spaces, F/OSS communities show they are welcoming women~\cite{PS6}. According to one interviewee from Calvo's~\cite{PS24} study, ``when you send things directly to women, they become a lot more involved". Women tend to hide their identities and gender to avoid bias and protect themselves~\cite{PS1}, but not in women-specific spaces, demonstrating they felt safe and comfortable in those spaces~\cite{PS48}.
%The benefit of women-specific forums was studied by Singh and Brandon~\cite{PS48}. Authors qualitatively analyzed 10,698 messages from five projects' mailing lists and found that the more active topics were women-focused events and activities, showing that these forums facilitates networking. Authors also found messages celebrating the successes of women and noticed that the majority of women used their names and affiliations in their signatures, demonstrating they felt safe and comfortable to reveal their identities. Having women speaking to women was also mentioned as a way ``to demystify the world of F/OSS"~\cite{PS6}. %Singh and Brandon~\cite{PS47} found that only 3\% of the 350 projects they analyzed have women-specific spaces, ranging from websites completely dedicated for women, women only IRC Channels, dedicated blogs, collection of resources for women in a blog post, dedicated Facebook pages or local meet-ups found that only 3\% of the 350 projects they analyzed have women-specific spaces, ranging from websites completely dedicated for women, women only IRC Channels, dedicated blogs, collection of resources for women in a blog post, dedicated Facebook pages or local meet-ups.
%Participants from Canedo et al.'s~\cite{PS6} study mentioned some specific initiatives (e.g., Outreachy\footnote{\label{foot7} Outreachy (\url{https://www.outreachy.org/}) is a paid, remote internship program that aims to support people from groups underrepresented in technology, such as women, helping newcomers to F/OSS to make their first contributions. Interns work with experienced mentors from F/OSS communities in a diverse set of activities, including code development, user experience, documentation, illustration, graphical design, or data science.  More than 90\% of past interns are women. } and local meetups) that might help to attract more women. Summer of Code events offer a diverse set of motivations and enhance the participants' sense of competence, autonomy, and relatedness, increasing the chances of future contributions as they internalize F/OSS projects' culture and values~\cite{silva2020theory}. Although it is pretty clear that women-specific spaces and events are essential to create safe spaces and make women comfortable, these spaces are still not commonplace---found in only 3\% of the 350 projects analyzed by Singh and Brandon~\cite{PS47}. Therefore, community building teams and maintainers must foster these kinds of efforts to make women start reporting to feel welcome and supported.

%\textbf{Codes of conduct: reward who follows, punish who violates.} Robson~\cite{PS34} concluded that it would make litter difference to have a code of conduct unless it is enforced among the project members. The authors showed no significant difference in the proportion of women contributing to projects with or without a code of conduct. Enforcing compliance with codes of conduct can be supported by tools like bots~\cite{PS8, wessel2018power}. Even though highly suggested by the literature as a strategy to increase inclusion, Singh and Brandon~\cite{PS47} found that only 8\% of the 355 sites of F/OSS projects that authors investigated have a code of conduct. To promote F/OSS projects to adopt a code of conduct, Prana et al.~\cite{PS16} suggested creating a reward program to recognize the projects that have one (e.g., GitHub could offer donation through sponsors, badges, etc.).
%Imtiaz et al. \cite{PS3} indicated that having the code of conduct might help to reduce the challenge of living with a \textsc{toxic culture} and the celebration may bring recognition and help to reduce the \texsc{impostor syndrome}'s feeling that women reported to face.

%\review{Although we found several strategies proposed in the literature, the level of evidence about their effectiveness is still weak.} 



